A High-Fidelity Simulation Framework for Grasping Stability Analysis in Human Casualty Manipulation

Recently, there has been a growing interest in rescue robots due to their vital role in addressing emergency scenarios and providing crucial support in challenging or hazardous situations where human intervention is difficult. However, very few of these robots are capable of actively engaging with humans and undertaking physical manipulation tasks. This limitation is largely attributed to the absence of tools that can realistically simulate physical interactions, especially the contact mechanisms between a robotic gripper and a human body. In this letter, we aim to address key limitations in current developments towards robotic casualty manipulation. Firstly, we present an integrative simulation framework for casualty manipulation. We adapt a finite element method (FEM) tool into the grasping and manipulation scenario, and the developed framework can provide accurate biomechanical reactions resulting from manipulation. Secondly, we conduct a detailed assessment of grasping stability during casualty grasping and manipulation simulations. To validate the necessity and superior performance of the proposed high-fidelity simulation framework, we conducted a qualitative and quantitative comparison of grasping stability analyses between the proposed framework and the state-of-the-art multi-body physics simulations. Through these efforts, we have taken the first step towards a feasible solution for robotic casualty manipulation.

==> content/case2.tex <==
\subsection{Case Study II: Human Limb Manipulation}
xxx \par

Since simulation of human manipulation with this level of fidelity (there's no the concept of ligament) is not achievable in a multi-body dynamics simulator. Thus, there is no meaningful qualitative and quantitative comparisons available. \par

==> content/related_work.tex <==
\section{Related Work}

\subsection{Robot-assisted Casualty Extraction and Evacuation} \label{ch:related-work-casualty-extraction-evacuation}

%Since the benefits of using a robot rescue system compare with a medic personnel are [xxx]. It is not surprising that army would be the major customer of such unmanned autonomous systems (UAS), therefore, sponsored researches of robot assisted casualty extraction and evacuation. Some representative systems of current state of casualty evacuation (CASEVAC) robots is presented below, and a more comprehensive review of search, extraction, evacuation, and medical field treatment robots can be find in \cite{extraction-review}. Please note that not all of the robotic systems presented below has victim extraction mechanisms, therefore, we will summarized and compare extraction mechanisms in Section~\ref{ch:related-work-victim-extraction}.

%[Valkyrie]
%As one of the earliest investigations on using mobile robot for the recovery of battlefield casualties. IROBOT CORP., at Somerville, MA, received research funding from the United States Department of Defense through SBIR (Small Business Innovation Research) project in 2003. \textbf{Valkyrie} was a patient recovery robot which is a modification of existing mobile platform and a flexible stretcher tethered to the robot. It can be remote operated by medic to approach to the patient and release the stretcher. The wounded soldier can then roll onto the stretcher and been dragged to a safe place. Valkyrie was targeted on injured person with assumptions that limbs are not seriously injured so that can still support body weight to adjust body pose and roll onto the stretcher. In addition, Valkyrie did not equipped with any actuated components to handle uneven terrain and to prevent the victim from flipping over while transporting. With these broad assumptions and limitations, Valkyrie was a successful exploration on using robot system on CASEVAC missions but still far from applicable in real-life. 

%[REX/REV]
%In 2003, another robotic patient recovery project was funded by DoD through SBIR. The award gave to Applied Perception Inc., Waxford PA. The outcome from this project was a "marsupial" extraction and evacuation vehicle (\textbf{REX/REV}) system. The REX was a small mobile robot for short range extraction, and it was loaded on the REV during system deployment ([Figure x.a REV]). When the system arrived near the victim, the REX ([Figure x.b REX]) was then approaching the victim itself with wheeled stretcher to load and drag the victim back to the REV for a faster transport to the nearest medical station. Compare to Valkyrie which was towing the stretcher on the ground, the REX equipped with a wheeled stretcher was more patient-friendly. 

%[BEAR]
%Instead of loading and transporting the victim using stretchers, the Battlefield Extraction Assist Robot (\textbf{BEAR}), developed by Vecna Robotics, took a different approach. As depicted in [Figure BEAR], BEAR was consist of a humanoid hydraulic torso and a mobile robot base, and it can carry the victim up to 500 pounds using the upper limbs and transporting with the tank car chassis. BEAR can be controlled remotely by medic personnel wearing a motion glove. Its abilities of operating in various environment and dynamically balancing make it stands out from other CASEVAC robots. 

%[RoNA]
%The Robotic Nursing Assistant, \textbf{RoNA}, was a humanoid robot designed to assist nurses in performing the labor intensive tasks such as lifting and repositioning patients around bed and transferring them from bed to bed \cite{RoNA}. RoNA is operating in a similar way as the \textbf{BEAR}, which is approaching to the patient and give him/her a lift. Although RoNA was initially a nursing robot, it has a combat variant for casualty extraction and evacuation for military uses. 

%[IWANO 2005]
%Other than direct military uses, some other groups of researchers focus on robot systems for rescue against nuclear disaster. Iwano Y., etal in 2005 proposed a group of small mobile robots to collaborate to rescue people in an area polluted with radioactive leakage in nuclear power institutions \cite{Iwano2005}. This traction robot system consists of many small mobile robots equipped with grippers and a stretcher robot. As depicted in [Figure Iwano20205], firstly, the small mobile robots with grippers push the four limbs of victim closer to the body, then they connect with the stretcher robot to slide under the victim and transfer to a safe place. The proposed robot system been built and conducted experimental study with a dummy doll on a flat concrete floor as a proof of concept. [need a sentence to conclude this paragraph]

%[Mark Yim 2011]

%\subsection{Methods of Victim Extraction}\label{ch:related-work-victim-extraction}

%When planning a casualty extraction and evacuation, how to approach to the victim and make physical contacts with him/her to either pull onto a stretcher or carry by arms of humanoid robot is the first and key question to mission success. However, almost none of the above mentioned robot systems are able to manage safe victim manipulation with minimum assumptions and without causing new injuries or aggregate the existing ones. In the following paragraphs, we will analysis some methods been used for casualty extraction and their limitations.

%[BEAR] [RoNA]
%In the example of the \textbf{BEAR} or \textbf{RoNA} that been discussed in Section~\ref{ch:related-work-casualty-extraction-evacuation}, the humanoid robot tries to mimic the most common approach that a human would take to carry someone. It slide their robot arms under the wounded soldier and lift. This seems to be very effective, however, it takes board assumptions that hard to be met in the case of casualty extraction. On one hand, the carrying motion inherently assumes the victim have both legs present and can hold his/her own weights. On the other hand, it can only safely carry the victim at lower limbs and back with assumptions that no head and neck trauma that required extra support during lifting and transporting. The lack of live evaluation of human body joint torques resulted from the casualty extraction motion can often lead in further injury to or death of the victim. 

%[IWANO 2005]
%need large space, need flat surface, only push and pull limbs, not lift. If obstacles, push/pull limb may overload joint torque.

%[Mark Yim 2011]

%[Some papers mentioned in Mark Yim 2011]

Since the benefits of using a robot rescue system compare with a medic personnel are [xxx], it is not surprising that army would be major customer of such unmanned autonomous systems (UAS), and therefore sponsored researches of robot assisted casualty extraction and evacuation. In this section, some representative systems of current state of casualty extraction and evacuation robots are presented as well as summarized in Table.X. A more comprehensive review of search, extraction, evacuation, and medical field treatment robots can be find in \cite{extraction-review}. \par

\begin{table*}[!ht]
	\centering
	\caption{example caption}
	\resizebox{\textwidth}{!}{%
	\begin{tabular}{@{}lllllll@{}}
		\toprule
		Name     & Category                                                          & Targeted Group                                                                                                                                                             & Autonomous? & \begin{tabular}[c]{@{}l@{}}Extraction \\ Safety \\ Evaluated?\end{tabular} & Manipulation Stability Evaluate?                                                                                         & Highlights                                                                                                                                                                                                                                    \\ \midrule
		Valkyrie & Evacuation                                                        & \begin{tabular}[c]{@{}l@{}}Injured person but not seriously\\ injured so that can still support\\ body weight to adjust body \\ pose and roll onto stretcher.\end{tabular} & No          & No                                                                         & \begin{tabular}[c]{@{}l@{}}No, it relays on patient to keep \\ balance during evacuation.\end{tabular}                   & \begin{tabular}[c]{@{}l@{}}One of the earliest investigation in \\ robot assisted evacuation mission.\end{tabular}                                                                                                                               \\
		REX-REV  & Evacuation                                                        & \begin{tabular}[c]{@{}l@{}}Injured person but not seriously \\ injured so that can still get on the \\ wheeled stretcher.\end{tabular}                                     & No          & No                                                                         & Similar to Valkyrie.                                                                                                     & \begin{tabular}[c]{@{}l@{}}One of the earliest investigation in \\ robot assisted evacuation mission. \\ Instead of towing on the ground as \\ Valkyrie did, REX had a wheeled \\ stretcher that is a bit more \\ patient-friendly.\end{tabular} \\
		BEAR     & \begin{tabular}[c]{@{}l@{}}Extraction, \\ Evacuation\end{tabular} & \begin{tabular}[c]{@{}l@{}}Wounded solider with no neck, \\ back, joint injury.\end{tabular}                                                                               & No          & No                                                                         & \begin{tabular}[c]{@{}l@{}}Partially, due to it is remotely \\ controlled by operator with \\ motion glove.\end{tabular} & \begin{tabular}[c]{@{}l@{}}First humanoid robot in robot assisted \\ extraction and evacuation.\end{tabular}                                                                                                                                     \\
		RoNA     & \begin{tabular}[c]{@{}l@{}}Extraction,\\ Evacuation\end{tabular}  & Similar to BEAR.                                                                                                                                                           & No          & No                                                                         & Similar to BEAR.                                                                                                         & \begin{tabular}[c]{@{}l@{}}Originally a nursing robot in assisting \\ repositioning patients on bed. Later \\ having a military version for \\ casualty extraction and evacuation.\end{tabular}                                                  \\ \bottomrule
	\end{tabular}%
}
\end{table*}

\begin{description}
	\item[Valkyrie]
\end{description}

In 2003, IROBOT CORP., at Somerville, MA, received research funding from the United States Department of Defense (DoD) through SBIR (Small Business Innovation Research)\cite{ValkyrieSBIR}. They developed \textbf{Valkyrie} as one of the earliest investigations on using mobile robot for the recovery of battlefield casualties.
% As one of the earliest investigations on using mobile robot for the recovery of battlefield casualties, IROBOT CORP., at Somerville, MA, received research funding from the United States Department of Defense (DoD) through SBIR (Small Business Innovation Research) in 2003 \cite{ValkyrieSBIR}.
Valkyrie, shown in Fig.~\ref{fig:casualty-extraction-robots}(a), is a patient recovery robot which is modified from an existing mobile platform, and a flexible stretcher tethered to the robot. It can be remote operated by a medic to approach to the patient and release the stretcher. The wounded soldier can then roll onto the stretcher and been dragged to a safe place. Valkyrie was targeted on injured person with assumptions that limbs are not seriously injured so that can still support body weight to adjust body pose and roll onto the stretcher. In addition, Valkyrie does not equipped with any actuated components to handle uneven terrain and to prevent the victim from flipping over while transporting. With these broad assumptions and limitations, Valkyrie is a successful exploration on using robot system on CASEVAC missions but still having limited application scenarios and far from applicable in real-life. \par

\begin{description}
	\item[REX-REV]
\end{description}

Another robotic patient recovery project was funded by DoD through SBIR \cite{REXREVsbir} in 2003. The award gave to Applied Perception Inc., Waxford PA. The outcome from this project is a "marsupial" extraction and evacuation vehicle (REX-REV) system \cite{Yoo2011}. The REX (Fig.~\ref{fig:casualty-extraction-robots}(b)) is a small mobile robot for short range extraction, and it is loaded on the REV (Fig.~\ref{fig:casualty-extraction-robots}(c)) during system deployment. When the system arrived near the victim, the REX  is then approaching the victim itself with wheeled stretcher to load and drag the victim back to the REV for a faster transport to the nearest medical station. Compare to Valkyrie which is towing the stretcher on the ground, the REX equipped with a wheeled stretcher is more patient-friendly. In table X, it is not categraized into the extraction robot because the robot seems not actively interact/manipulate human body directly. \par

\begin{description}
	\item[BEAR]
\end{description}

Instead of loading and transporting the victim using stretchers, the Battlefield Extraction Assist Robot (BEAR), developed by Vecna Robotics, took a different approach. As depicted in Fig.~\ref{fig:casualty-extraction-robots}(e), BEAR consists of a humanoid hydraulic torso and a mobile robot base, and it can carry the victim up to 500 pounds using the upper limbs and transporting with the tank car chassis. BEAR can be controlled remotely by a medic personnel wearing a motion glove. Its abilities of operating in various environment and dynamically balancing make it stands out from other casualty extraction robots. \par
In the example of the BEAR system, the humanoid robot tries to mimic the most common approach that a human would take to carry someone. It slides its robot arms under the wounded soldier and lift. This seems to be very effective, however, it takes board assumptions that are hard to be met in the case of casualty extraction. On one hand, the carrying motion inherently assumes the victim have both legs present and can hold his/her own weights. On the other hand, it can only safely carry the victim at lower limbs and back with assumptions that no head and neck trauma that required extra support during lifting and transporting. Otherwise, the head and neck trauma can become life-threatening issues immediately. \par
% The lack of live evaluation of human body joint torques resulted from the casualty extraction motion can often lead in further injury to or death of the victim. \pars

\begin{description}
	\item[RoNA]
\end{description}

The Robotic Nursing Assistant, RoNA, shown in Fig.~\ref{fig:casualty-extraction-robots}(f), was a humanoid robot designed to assist nurses in performing the labor intensive tasks such as lifting and repositioning patients around bed and transferring them from bed to bed \cite{RoNA}. RoNA is operating in a similar way as the BEAR, which it approaches to the patient and gives him/her a lift. Although RoNA is initially a nursing robot, it has a combat variant for casualty extraction and evacuation for military uses. It shares the same limitations with the BEAR system discussed above. \par

%\begin{description}
%	\item[Traction Robot System]
%\end{description}

%[IWANO 2005]
%Other than direct military uses, some other groups of researchers focus on robot systems for rescue against nuclear disaster. Iwano Y., etal in 2005 proposed a group of small mobile robots to collaborate to rescue people in an area polluted with radioactive leakage in nuclear power institutions \cite{Iwano2005}. This traction robot system consists of many small mobile robots equipped with grippers and a stretcher robot. As depicted in [Figure Iwano2005], firstly, the small mobile robots with grippers push the four limbs of victim closer to the body, then they connect with the stretcher robot to slide under the victim and transfer to a safe place. \par 
%The initial prototype was built, and an experimental study was conducted with a dummy doll as a proof of concept. Its operation needs a large flat surface with the dummy doll lie down in the center of floor. The robot system requires a large flat surface to operate, which limits its practical field of applications. In addition, during body pose manipulation, xxx.

\begin{description}
	\item[Others]
\end{description}

In addition to robot systems that try to address the casualty extraction and evacuation missions by themselves, other projects focuses on developing some mobile robots that being small enough but can still be beneficial to the victim manipulation tasks. \cite{Yim2009} designed small mobile robot platforms that equipped with special cufflets and foam dispensers to assist in victim limbs manipulation and head/neck stabilization (Fig.~\ref{fig:casualty-extraction-robots}(g)). \cite{Iwano2005postureManipulation} also worked on a small mobile platform with cufflet-like robotic hand attached to perform victim posture manipulation, depicted in Fig.~\ref{fig:casualty-extraction-robots}(h). 


\myparagraph{Discussion}
When planning a casualty extraction and evacuation, how to approach to the victim and make physical contacts with him/her to either pull on to a stretcher or carry by arms of humanoid robot is the first and key questions to mission success. However, most of the above mentioned robot systems are experimental based, and none of them are able to ensure safe victim manipulation with minimum assumptions and without causing new injuries or aggregate the existing ones. The lack of simulation tools to provide high-fidelity victim manipulations is the missing puzzle of safe casualty extraction missions. In the content of this work, we presents a simulation framework for robot-assisted victim manipulation and casualty extraction, as well as associated grasping stability analysis. \par
% When planning a casualty extraction and evacuation, how to approach to the victim and make physical contacts with him/her to either pull onto a stretcher or carry by arms of humanoid robot is the first and key question to mission success. However, most of the above mentioned robot systems are experimental based, and none of them are able to ensure safe victim manipulation with minimum assumptions and without causing new injuries or aggregate the existing ones. The lack of simulation tools to provide high-fidelity victim manipulations is the missing puzzle of safe casualty extraction missions. This is exactly what we are contributing on. Before proposing our approach, Section~\ref{ch:related-work-robot-simulation-tools} will introduce some existing robot simulation tools that will be utilized. \par 

\subsection{Robot Simulation Tools} \label{ch:related-work-robot-simulation-tools}

\QZComment{Need a transition paragraph.}

Here we discuss two types of simulation tools that focus on robot systems development for distinct applications. 

%The most widely used simulation tools in robotics community is multi-body dynamics simulator, having ROS Gazebo as a well-known example. [Pros: real-time motion planning and simulation, real-time contact force computed] [Cons: light in computing power, rigid-body contact, point contact, unrealistic in many cases]. 

%FEM [Pros: deal with soft contact, deformeable object, realistic] [Cons: compulational expansive, overly complicated/not needed for many robotics development, e.g. mobile robot, robot manipulators in industrial settings.]


%Most of the existing simulation tools in robotics can be categorized into three classes: (a) physics-based rigid body simulator, (b) finite element method (FEM), and (c) human motion modeling software. Each group have their unique focus and advantages, and individually, each group have been effective in solving specific problems, which is reviewed as the following. \par

%\myparagraph{Class (a)} 
\begin{description}
	\item[Multi-body Dynamics Simulator]
\end{description}

Multi-body dynamics simulators are the most widely used tool for modeling and simulation within the robotics community. Gazebo \cite{Gazebo} belongs to this category, along with MuJoCo \cite{MuJoCo} and many more \cite{Unity3D-MATLAB-Simulator,ROSUnitySim}. In these multi-body dynamics simulators, robots and objects are represented as a spatial tree of links and joints. Each joint can be controlled individually, and collisions and contacts are computed efficiently within any pair of the defined geometries. Since this set of simulation tools treat objects as rigid bodies, the processing speed is fast, which can accommodate real-time applications, with a cost of simulation fidelity. \par

%they support research involving \myhigh{simulation of robotic manipulation}

%\myparagraph{Class (b)} 
\begin{description}
	\item[Finite-Element Method]
\end{description}

A higher-fidelity simulation tool is the finite-element method (FEM). It is a numerical technique designed for simulations involving deformable objects, and many recent FEM works are capable of providing high-fidelity anatomical representations of human body. 
%
For example, a practical and simplified complete human body FE model was developed and applied to the evaluation of crash safety of a vehicle \cite{Watanabe2001Toyota,Iwamoto2002THUMS-Toyota}, and the model was based on FE models of the parts of the human body which can predict localized injuries. More recently, high-fidelity human brain models have been developed, with the help of computed tomography (CT) and magnetic resonance imaging (MRI) technologies. Researchers investigate traumatic brain injuries \cite{Yang2014FEM-head-injury} and provide recommendations to personal protective equipment manufacturers \cite{Levadnyi2018FEM-head-injury}. Traditional finite element modeling techniques coupled with a contact solver have the potential to provide high-fidelity anatomical deformation and kinematic data for a variety of loading conditions. \par

%Class~(b) contributes to \myhigh{the simulation of the human body}. 

%\myparagraph{Class (c)} Human motion modeling software tools are commonly used for biomechanical simulations and analysis, and they support development in certain areas of robotics by accurately capturing human motion. This class also contributes to \myhigh{the simulation of the human body}, with OpenSim \cite{OpenSim} being an example. In conjunction with commercially available motion capture systems, OpenSim has been widely used in computing joint angles to evaluate the risks associated to the musculoskeletal disorders for the upper limbs \cite{Do2019,Panariello2019}, and in human gait analysis \cite{Yu2020gait,Wang2018gait}. Software like OpenSim specializes in creating musculoskeletal models and performing kinematic and dynamic analysis to estimate internal loading of the musculoskeletal system. \par

\myparagraph{Discussion}
To develop a simulation framework for robot-assisted casualty extraction, we utilize the strength of multi-body dynamics simulator on simulating robot motion and the strength of FEM on simulating deformable human body. Our proposed simulation framework and grasping stability analysis will be presented in \QZComment{update sections.}\par



==> figures/psfragFmt/pdfGen_preamble_psfrag.tex <==
%%  common packages needed
\usepackage{graphicx}
\usepackage{epsfig}  %for using eps figures
\usepackage{psfrag}  %for enabling use of psfrag commands
%\usepackage[T1]{fontenc}
\usepackage{amsmath}
\usepackage[e]{esvect} % beautiful vector \vv{AB}
\newcommand {\mb}[1]{\mathbf{#1}} % all replaced
\newcommand {\bs}[1]{\boldsymbol{#1}}
\newcommand{\uvec}[1]{\hat{\mathbf{#1}}}  %defines a macro for writing unit vectors
\newcommand{\uvecf}[3]{\,^{#1}\hat{\mathbf{#2}}_{#3}}
\newcommand{\T}{^{\mathrm{T}}}  %shortcut for transpose
\usepackage{color}  %needed for color text
\newcommand{\green}[1]{\textcolor[rgb]{0.00,1.00,0.00}{#1}}
\newcommand{\red}[1]{\textcolor[rgb]{1.00,0.00,0.00}{#1}}
\newcommand{\blue}[1]{\textcolor[rgb]{0.00,0.00,1.00}{#1}}   %for marking sentences that need changes
%%  page size and font setup

==> figures/psfragFmt/tikz_circled.tex <==
% The use of tikz seems to generate an empty second page ...
% However, when including a pdf figure, the second empty page seems to not matter, so, use this preamble when you need the circled command in a figure.
\usepackage{tikz}
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,draw,inner sep=1pt] (char) {#1};}}
